PENELLOPE IV. A comparison between optical forbidden lines and $\rm H_2$ UV lines in the Orion OB1b and $\sigma$-Ori associations

Observing the spatial distribution and excitation processes of atomic and molecular gas in the inner regions (< 20 au) of young (< 10 Myr) protoplanetary disks helps us to understand the conditions for the formation and evolution of planetary systems. In the framework of the PENELLOPE and ULLYSES projects, we aim to characterize the atomic and molecular component of protoplanetary disks in a sample of 11 Classical T Tauri Stars (CTTs) of the Orion OB1 and $\sigma$-Orionis associations. We analyzed the flux-calibrated optical-forbidden lines and the fluorescent ultraviolet $\rm H_2$ progressions using spectra acquired with ESPRESSO at VLT, UVES at VLT and HST-COS. Line morphologies were characterized through Gaussian decomposition. We then focused on the properties of the narrow low-velocity (FWHM < 40 $km$ $s^{-1}$ and |$v_p$| < 30 $km$ $s^{-1}$) component (NLVC) of the [OI] 630 nm line, compared with the properties of the UV-$\rm H_2$ lines. We found that the [OI]630 NLVC and the UV-$\rm H_2$ lines are strongly correlated in terms of peak velocities, full width at half maximum, and luminosity. The luminosities of the [OI]630 NLVC and UV-$\rm H_2$ correlate with the accretion luminosity with a similar slope, as well as with the luminosity of the CIV 154.8, 155 nm doublet. We discuss such correlations in the framework of the currently suggested excitation processes for the [OI]630 NLVC. Our results can be interpreted in a scenario in which the [OI]630 NLVC and UV-$\rm H_2$ have a common disk origin with a partially overlapped radial extension. We also suggest that the excitation of the [OI] NLVC is mainly induced by stellar FUV continuum photons more than being of thermal origin. This study demonstrates the potential of contemporaneous wide-band high-resolution spectroscopy in linking different tracers of protoplanetary disks.

==> Tables/Journal_Observations.tex <==
\begin{table*}
\small
\center
\caption{\label{tab:journal} Journal of Observations}
\begin{tabular}{l|ll|l|l}
\hline
\hline
Name    & epoch     & HJD       & \multicolumn{2}{c}{Instrument} 	\\
        &           & 2459100+  & OPTICAL       & UV 			    \\
\hline
CVSO58	& ep1  		& 83.61246	& UVES			&					\\ 
CVSO58	& ep2  		& 84.61185	& UVES			&					\\ 
CVSO58	& ep3  		& 85.60270	& UVES			&					\\ 
CVSO58	& ep3  		& 85.76194	& X-Shooter		&					\\ 
\hline
CVSO90	& ep1  		& 			&				&					\\ 
CVSO90	& ep2  		&			&				&					\\ 
CVSO90	& ep3  		&			&				&					\\ 
\hline
CVSO104	& ep1  		&			&				&					\\ 
CVSO104	& ep2  		&			&				&					\\ 
CVSO104	& ep3  		&			&				&					\\ 
\hline
CVSO107	& ep1  		& 86.66418	& UVES			&					\\ 
CVSO107	& ep2  		& 87.58635	& X-Shooter		&					\\ 
CVSO107	& ep2  		& 87.60273	& UVES			&					\\ 
CVSO107	& ep3  		& 88.65286	& UVES			&					\\ 
\hline
CVSO109	& ep1  		& 79.65665	& UVES			&					\\ 
CVSO109	& ep2  		& 80.63793	& UVES			&					\\ 
CVSO109	& ep3  		& 81.65721	& X-Shooter		&					\\ 
CVSO109	& ep3  		& 81.67743	& UVES			&					\\ 
\hline
CVSO146	& ep1  		& 92.62465	& ESPRESSO		&					\\ 
CVSO146	& ep2  		& 93.60337	& ESPRESSO		&					\\ 
CVSO146	& ep3  		& 94.58387	& X-Shooter		&					\\ 
CVSO146	& ep3  		& 94.59294	& ESPRESSO		&					\\ 
\hline
CVSO165	& ep1  		& 96.57902	& ESPRESSO		&					\\ 
CVSO165	& ep2  		& 97.58384	& X-Shooter		&					\\ 
CVSO165	& ep2  		& 97.60896	& ESPRESSO		&					\\ 
CVSO165	& ep3  		& 98.61706	& ESPRESSO		&					\\ 
\hline
CVSO176	& ep1  		& 85.68282	& X-Shooter		&					\\ 
CVSO176	& ep1  		& 87.68387	& UVES			&					\\ 
CVSO176	& ep2  		& 88.61053	& UVES			&					\\ 
CVSO176	& ep3  		& 89.59468	& UVES			&					\\ 
\hline
\hline
SO518	& ep1  		& 82.66445	& UVES			&					\\ 
SO518	& ep2  		& 83.70244	& UVES			&					\\ 
SO518	& ep3  		& 84.65642	& UVES			&					\\ 
SO518	& ep3  		& 85.64623	& X-Shooter		&					\\ 
\hline
SO583	& ep1  		& 82.68932	& UVES			&					\\ 
SO583	& ep2  		& 83.64056	& UVES			&					\\ 
SO583	& ep3  		& 84.63973	& UVES			&					\\ 
SO583	& ep3  		& 85.66222	& X-Shooter		&					\\ 
\hline
SO1153	& ep1  		& 90.70681	& X-Shooter		&					\\ 
SO1153	& ep1  		& 91.83202	& UVES			&					\\ 
SO1153	& ep2  		& 92.59172	& UVES			&					\\ 
SO1153	& ep3  		& 93.63656	& UVES			&					\\ 
\hline
\end{tabular}
\end{table*} 

